Inherent Limits on Topology-Based Link Prediction

Link prediction systems (e.g. recommender systems) typically use graph topology as one of their main sources of information. However, automorphisms and related properties of graphs beget inherent limits in predictability. We calculate hard upper bounds on how well graph topology alone enables link prediction for a wide variety of real-world graphs. We find that in the sparsest of these graphs the upper bounds are surprisingly low, thereby demonstrating that prediction systems on sparse graph data are inherently limited and require information in addition to the graph topology.

==> figures/data/US_500_airports_u_k-all_ref-0.1_nef-1.0_he-true_raw_AUPR_average_points.tex <==
\pgfplotstableread{
k	AUPR	confintwidth	label
1.002500	0.999899	0.000331	1
}{\USFiveOhOhairportsukallrefOhOnenefOneOhhetruerawAUPRaveragepoints}

==> figures/data/US_500_airports_u_k-all_ref-0.1_nef-1.0_he-true_raw_AUPR_raw_points.tex <==
\pgfplotstableread{
k	AUPR	label
1.017797	0.999607	1
1.002366	0.999994	1
0.987614	0.999995	1
0.981818	1.000000	1
1.112680	0.999971	2
1.103268	0.999994	2
1.078964	0.999995	2
1.077541	1.000000	2
}{\USFiveOhOhairportsukallrefOhOnenefOneOhhetruerawAUPRrawpoints}

==> figures/data/US_airports_2010_u_k-all_ref-0.1_nef-1.0_he-true_raw_AUPR_average_points.tex <==
\pgfplotstableread{
k	AUPR	confintwidth	label
1.002500	0.999613	0.000224	1
}{\USairportsTwoOhOneOhukallrefOhOnenefOneOhhetruerawAUPRaveragepoints}

==> figures/data/US_airports_2010_u_k-all_ref-0.1_nef-1.0_he-true_raw_AUPR_raw_points.tex <==
\pgfplotstableread{
k	AUPR	label
1.002530	0.999694	1
0.983819	0.999532	1
1.117558	0.999707	2
1.111612	0.999604	2
}{\USairportsTwoOhOneOhukallrefOhOnenefOneOhhetruerawAUPRrawpoints}

==> figures/data/celegans_m_k-all_ref-0.1_nef-auto_he-false_raw_AUPR_average_points.tex <==
\pgfplotstableread{
k	AUPR	confintwidth	label
1.002500	1.000000	0.000000	1
}{\celegansmkallrefOhOnenefautohefalserawAUPRaveragepoints}

==> figures/data/citeseer_k-all_ref-0.1_nef-1.0_he-true_raw_AUPR_average_points.tex <==
\pgfplotstableread{
k	AUPR	confintwidth	label
1.010000	0.488472	0.024465	1
2.000000	0.666285	0.022483	1
3.000000	0.700967	0.024245	1
4.000000	0.703214	0.024752	1
}{\citeseerkallrefOhOnenefOneOhhetruerawAUPRaveragepoints}

==> figures/data/collins_yeast_k-all_ref-0.1_nef-1.0_he-true_raw_AUPR_average_points.tex <==
\pgfplotstableread{
k	AUPR	confintwidth	label
1.005000	0.968823	0.023219	1
2.000000	0.977928	0.017317	1
}{\collinsyeastkallrefOhOnenefOneOhhetruerawAUPRaveragepoints}

==> figures/data/collins_yeast_k-all_ref-0.1_nef-1.0_he-true_raw_AUPR_raw_points.tex <==
\pgfplotstableread{
k	AUPR	label
0.987872	0.960446	1
1.024455	0.977200	1
1.988711	0.971680	1
1.985110	0.984175	1
2.115932	0.973402	2
2.116159	0.986203	2
}{\collinsyeastkallrefOhOnenefOneOhhetruerawAUPRrawpoints}

==> figures/data/convote_k-all_ref-0.1_nef-auto_he-false_raw_AUPR_average_points.tex <==
\pgfplotstableread{
k	AUPR	confintwidth	label
1.005000	0.988249	0.006673	1
2.000000	0.990603	0.006192	1
}{\convotekallrefOhOnenefautohefalserawAUPRaveragepoints}

==> figures/data/cora_k-all_ref-0.1_nef-1.0_he-true_raw_AUPR_average_points.tex <==
\pgfplotstableread{
k	AUPR	confintwidth	label
1.007500	0.668171	0.021308	1
2.000000	0.902855	0.013333	1
3.000000	0.914460	0.013881	1
}{\corakallrefOhOnenefOneOhhetruerawAUPRaveragepoints}

==> figures/data/eucore_k-all_ref-0.1_nef-1.0_he-true_raw_AUPR_average_points.tex <==
\pgfplotstableread{
k	AUPR	confintwidth	label
1.002500	0.999890	0.000060	1
}{\eucorekallrefOhOnenefOneOhhetruerawAUPRaveragepoints}

==> figures/data/eucore_k-all_ref-0.1_nef-1.0_he-true_raw_AUPR_raw_points.tex <==
\pgfplotstableread{
k	AUPR	label
1.027175	0.999894	1
1.011200	0.999939	1
0.985506	0.999863	1
0.984851	0.999865	1
1.096761	0.999906	2
1.114592	0.999943	2
1.091960	0.999875	2
1.078589	0.999923	2
}{\eucorekallrefOhOnenefOneOhhetruerawAUPRrawpoints}

==> figures/data/faculty_comp_sci_k-all_ref-0.1_nef-1.0_he-true_raw_AUPR_average_points.tex <==
\pgfplotstableread{
k	AUPR	confintwidth	label
1.002500	1.000000	0.000000	1
}{\facultycompscikallrefOhOnenefOneOhhetruerawAUPRaveragepoints}

==> figures/data/faculty_comp_sci_k-all_ref-0.1_nef-1.0_he-true_raw_AUPR_raw_points.tex <==
\pgfplotstableread{
k	AUPR	label
0.999353	1.000000	1
1.025889	1.000000	1
1.109151	1.000000	2
1.082639	1.000000	2
}{\facultycompscikallrefOhOnenefOneOhhetruerawAUPRrawpoints}

==> figures/data/foodweb_k-all_ref-0.1_nef-auto_he-false_raw_AUPR_average_points.tex <==
\pgfplotstableread{
k	AUPR	confintwidth	label
1.002500	1.000000	0.000000	1
}{\foodwebkallrefOhOnenefautohefalserawAUPRaveragepoints}

==> figures/data/highschool_k-all_ref-0.1_nef-auto_he-false_raw_AUPR_average_points.tex <==
\pgfplotstableread{
k	AUPR	confintwidth	label
1.002500	1.000000	0.000000	1
}{\highschoolkallrefOhOnenefautohefalserawAUPRaveragepoints}

==> figures/data/innovation_k-all_ref-0.1_nef-auto_he-false_raw_AUPR_average_points.tex <==
\pgfplotstableread{
k	AUPR	confintwidth	label
1.002500	0.999938	0.000235	1
}{\innovationkallrefOhOnenefautohefalserawAUPRaveragepoints}

==> figures/data/jazz_collab_k-all_ref-0.1_nef-1.0_he-true_raw_AUPR_average_points.tex <==
\pgfplotstableread{
k	AUPR	confintwidth	label
1.002500	1.000000	0.000000	1
}{\jazzcollabkallrefOhOnenefOneOhhetruerawAUPRaveragepoints}

==> figures/data/jazz_collab_k-all_ref-0.1_nef-1.0_he-true_raw_AUPR_raw_points.tex <==
\pgfplotstableread{
k	AUPR	label
0.988802	1.000000	1
1.009074	1.000000	1
1.088015	0.998209	2
1.103697	0.997648	2
}{\jazzcollabkallrefOhOnenefOneOhhetruerawAUPRrawpoints}

==> figures/data/mysql_calls_k-all_ref-0.1_nef-1.0_he-true_raw_AUPR_average_points.tex <==
\pgfplotstableread{
k	AUPR	confintwidth	label
1.005000	0.860292	0.034537	1
2.000000	0.958124	0.033351	1
}{\mysqlcallskallrefOhOnenefOneOhhetruerawAUPRaveragepoints}

==> figures/data/mysql_calls_k-all_ref-0.1_nef-1.0_he-true_raw_AUPR_raw_points.tex <==
\pgfplotstableread{
k	AUPR	label
1.013271	0.860770	1
1.022568	0.834513	1
0.990462	0.861607	1
1.025351	0.884281	1
1.990607	0.962819	1
2.023567	0.941233	1
1.998977	0.944519	1
1.992752	0.983925	1
2.076594	0.966075	2
2.102078	0.945247	2
2.075272	0.946859	2
2.100400	0.986719	2
}{\mysqlcallskallrefOhOnenefOneOhhetruerawAUPRrawpoints}

==> figures/data/powergrid_k-all_ref-0.1_nef-1.0_he-true_raw_AUPR_average_points.tex <==
\pgfplotstableread{
k	AUPR	confintwidth	label
1.017500	0.112928	0.012454	1
2.000000	0.438536	0.021539	1
3.000000	0.617305	0.020970	1
4.000000	0.686040	0.020707	1
5.000000	0.707751	0.022235	1
6.000000	0.713412	0.022595	1
7.000000	0.713984	0.022833	1
}{\powergridkallrefOhOnenefOneOhhetruerawAUPRaveragepoints}

==> figures/data/roget_thesaurus_k-all_ref-0.1_nef-1.0_he-true_raw_AUPR_average_points.tex <==
\pgfplotstableread{
k	AUPR	confintwidth	label
1.005000	0.989118	0.006376	1
2.000000	0.999921	0.000102	1
}{\rogetthesauruskallrefOhOnenefOneOhhetruerawAUPRaveragepoints}

==> figures/data/roget_thesaurus_k-all_ref-0.1_nef-1.0_he-true_raw_AUPR_raw_points.tex <==
\pgfplotstableread{
k	AUPR	label
1.012229	0.992165	1
0.998312	0.989826	1
1.024694	0.983670	1
0.998538	0.990812	1
1.982204	1.000000	1
2.016532	0.999870	1
1.982675	0.999879	1
2.020051	0.999936	1
2.117118	1.000000	2
2.087517	0.999898	2
2.088482	0.999948	2
2.086548	0.999966	2
}{\rogetthesauruskallrefOhOnenefOneOhhetruerawAUPRrawpoints}

==> figures/data/roman_roads_u_k-all_ref-0.1_nef-1.0_he-true_raw_AUPR_average_points.tex <==
\pgfplotstableread{
k	AUPR	confintwidth	label
1.005000	0.888279	0.030678	1
2.000000	0.997738	0.002297	1
}{\romanroadsukallrefOhOnenefOneOhhetruerawAUPRaveragepoints}

==> figures/data/roman_roads_u_k-all_ref-0.1_nef-1.0_he-true_raw_AUPR_raw_points.tex <==
\pgfplotstableread{
k	AUPR	label
0.990628	0.899347	1
1.028578	0.877212	1
1.988954	0.998567	1
1.998163	0.996910	1
2.124273	0.999563	2
2.076768	0.999495	2
}{\romanroadsukallrefOhOnenefOneOhhetruerawAUPRrawpoints}

==> figures/data/species_1_brain_k-all_ref-0.1_nef-1.0_he-true_raw_AUPR_average_points.tex <==
\pgfplotstableread{
k	AUPR	confintwidth	label
1.002500	1.000000	0.000000	1
}{\speciesOnebrainkallrefOhOnenefOneOhhetruerawAUPRaveragepoints}

==> figures/data/species_1_brain_k-all_ref-0.1_nef-1.0_he-true_raw_AUPR_raw_points.tex <==
\pgfplotstableread{
k	AUPR	label
0.995941	1.000000	1
1.017138	1.000000	1
0.995980	1.000000	1
0.998515	1.000000	1
1.119158	1.000000	2
1.101512	1.000000	2
1.104898	1.000000	2
1.110321	1.000000	2
}{\speciesOnebrainkallrefOhOnenefOneOhhetruerawAUPRrawpoints}

==> figures/data/y2h_ppi_k-all_ref-0.1_nef-1.0_he-true_raw_AUPR_average_points.tex <==
\pgfplotstableread{
k	AUPR	confintwidth	label
1.007500	0.434241	0.023568	1
2.000000	0.616794	0.031216	1
3.000000	0.633552	0.032002	1
}{\yTwohppikallrefOhOnenefOneOhhetruerawAUPRaveragepoints}

==> figures/limits_over_k_figure_old.tex <==
\input{figures/data/cora_k-all_ref-0.05_nef-auto_he-false_raw_AUPR_average_points_noinf}
\input{figures/data/cora_k-all_ref-0.05_nef-auto_he-false_raw_AUPR_raw_points}
%		\addplot[scatter,only marks,%
%			scatter src=explicit symbolic]%
%		table[meta=label] {\randcorakallrefOhOhFivenefautohetruerawAUPRrawpoints};

%		\addplot[brown,thick,mark=x, error bars/.cd,y explicit,y dir=both]
%		table [x index=0,y index=1,y error index=2] {\randcorakallrefOhOhFivenefautohetruerawAUPRaveragepoints};

\input{figures/data/citeseer_k-all_ref-0.05_nef-auto_he-false_raw_AUPR_average_points_noinf}
\input{figures/data/citeseer_k-all_ref-0.05_nef-auto_he-false_raw_AUPR_raw_points}

\input{figures/data/y2h_ppi_k-all_ref-0.1_nef-1.0_he-true_raw_AUPR_average_points_noinf}
\input{figures/data/y2h_ppi_k-all_ref-0.1_nef-1.0_he-true_raw_AUPR_raw_points}

\input{figures/data/powergrid_k-all_ref-0.1_nef-1.0_he-true_raw_AUPR_average_points_noinf}
\input{figures/data/powergrid_k-all_ref-0.1_nef-1.0_he-true_raw_AUPR_raw_points}

\begin{tabular}{ll}
	\textbf{\ \ Results on Cora ML Citation Network} & \textbf{\ \ Results on Citeseer Citation Network} \\
	\begin{tikzpicture}[scale=0.9]
		\begin{axis}[%	
		scatter/classes={%
			0={mark=square*,blue},%
			1={mark=triangle,black},%
			2={mark=none,draw=none},%
			3={mark=square*,brown},%
			4={mark=o,brown},%
			5={mark=o,draw=brown}},%
		xlabel=Number of Hops ($k$) of Information,%
		ylabel=Upper Bound on AUPR Score,%
		ymin=0,ymax=1]
		\addplot[scatter,only marks,%
			scatter src=explicit symbolic]%
		table[meta=label] {\corakallrefOhOhFivenefautohefalserawAUPRrawpoints};
		\addplot[black,thick,mark=x, error bars/.cd,y explicit,y dir=both]
		table [x index=0,y index=1,y error index=2] {\corakallrefOhOhFivenefautohefalserawAUPRaveragepoints};
		\end{axis}
	\end{tikzpicture} &
	\begin{tikzpicture}[scale=0.9]
		\begin{axis}[%	
		scatter/classes={%
			0={mark=square*,blue},%
			1={mark=triangle,black},%
			2={mark=none,draw=none},%
			3={mark=square*,brown},%
			4={mark=o,brown},%
			5={mark=o,draw=brown}},%
		xlabel=Number of Hops ($k$) of Information,%
		ylabel=Upper Bound on AUPR Score,%
		ymin=0,ymax=1]
		\addplot[scatter,only marks,%
			scatter src=explicit symbolic]%
		table[meta=label] {\citeseerkallrefOhOhFivenefautohefalserawAUPRrawpoints};
		\addplot[black,thick,mark=x, error bars/.cd,y explicit,y dir=both]
		table [x index=0,y index=1,y error index=2] {\citeseerkallrefOhOhFivenefautohefalserawAUPRaveragepoints};
		\end{axis}
	\end{tikzpicture} \\
	\ & \ \\
		\textbf{\ \ Results on USA Powergrid Network} & \textbf{\ \ Results on Y2H PPI Network} \\
		\begin{tikzpicture}[scale=0.9]
		\begin{axis}[%	
		scatter/classes={%
			0={mark=square*,blue},%
			1={mark=triangle,black},%
			2={mark=none,draw=none},%
			3={mark=square*,brown},%
			4={mark=o,brown},%
			5={mark=o,draw=brown}},%
		xlabel=Number of Hops ($k$) of Information,%
		ylabel=Upper Bound on AUPR Score,%
		ymin=0,ymax=1]
		\addplot[scatter,only marks,%
			scatter src=explicit symbolic]%
		table[meta=label] {\powergridkallrefOhOnenefOneOhhetruerawAUPRrawpoints};
		\addplot[black,thick,mark=x, error bars/.cd,y explicit,y dir=both]
		table [x index=0,y index=1,y error index=2] {\powergridkallrefOhOnenefOneOhhetruerawAUPRaveragepoints};
		\end{axis}
	\end{tikzpicture} &
	\begin{tikzpicture}[scale=0.9]
		\begin{axis}[%	
		scatter/classes={%
			0={mark=square*,blue},%
			1={mark=triangle,black},%
			2={mark=none,draw=none},%
			3={mark=square*,brown},%
			4={mark=o,brown},%
			5={mark=o,draw=brown}},%
		xlabel=Number of Hops ($k$) of Information,%
		ylabel=Upper Bound on AUPR Score,%
		ymin=0,ymax=1]
		\addplot[scatter,only marks,%
			scatter src=explicit symbolic]%
		table[meta=label] {\yTwohppikallrefOhOnenefOneOhhetruerawAUPRrawpoints};
		\addplot[black,thick,mark=x, error bars/.cd,y explicit,y dir=both]
		table [x index=0,y index=1,y error index=2] {\yTwohppikallrefOhOnenefOneOhhetruerawAUPRaveragepoints};
		\end{axis}
	\end{tikzpicture}
	\end{tabular}

==> figures/lp_limits_intro_figure_horizontal_backup.tex <==
\begin{tikzpicture}[scale=0.7]

% Left side
\begin{scope}[shift={(1,-0.5)}]
\node [basicnode] (v4) at (-3.5,2.5) {};
\node [basicnode] (v2) at (-2,2.5) {};
\node [basicnode] (v5) at (-3,4) {};
\node [basicnode] (v6) at (-1.5,4) {};
\node [basicnode] (v1) at (-3.5,1) {};
\node [basicnode] (v3) at (-2,1) {};
\draw [basicedge] (v1) edge (v2);
\draw [basicedge] (v3) edge (v4);
\draw [basicedge] (v3) edge (v2);
\draw [basicedge] (v4) edge (v2);
\draw [basicedge] (v2) edge (v5);
\draw [basicedge] (v2) edge (v6);
\draw [basicedge] (v5) edge (v6);

\draw [highlightededge] (v5) edge (v4);
\draw [highlightededge] (v4) edge (v1);
\draw [highlightededge] (v1) edge (v3);
\end{scope}


\begin{scope}[shift={(6.5,5)}]
\node [basicnode] (v9) at (-2.5,-3.5) {};
\node [basicnode] (v10) at (-2.5,-2) {};
\node [basicnode] (v11) at (-0.5,-3) {};
\node [basicnode] (v12) at (-0.5,-4) {};
\node [basicnode] (v8) at (-4.5,-4) {};
\node [basicnode] (v7) at (-4.5,-3) {};


\draw [basicedge] (v7) edge (v8);
\draw [basicedge] (v8) edge (v9);
\draw [basicedge] (v9) edge (v7);
\draw [basicedge] (v9) edge (v10);
\draw [basicedge] (v9) edge (v11);
\draw [basicedge] (v9) edge (v12);
\draw [basicedge] (v12) edge (v11);
\end{scope}

% Dividers
\begin{scope}[shift={(-0.25,0)}]
\node [blanknode] (v15) at (1.5,5.5) {};
\node [blanknode] (v16) at (1.5,-0.5) {};
\draw (v15) edge (v16);
\end{scope}

\begin{scope}[shift={(5.25,0)}]
\node [blanknode] (v15) at (1.5,5.5) {};
\node [blanknode] (v16) at (1.5,-0.5) {};
\draw (v15) edge (v16);
\end{scope}

% Text nodes
\node [textnode] at (-1.5,5) {Original Graph with};
\node [textnode] at (-1.5,4.5) {Three Hidden Links};

\node [textnode] at (4,5) {Same Network with the};
\node [textnode] at (4,4.5) {Three Links Removed};

\node [textnode] at (13,5) {Three of Eight Equally};
\node [textnode] at (13,4.5) {Valid Reconstructions};

% Right side
\begin{scope}[shift={(12,6.75)}]
\node [basicnode] (v9) at (-2.5,-3.5) {};
\node [basicnode] (v10) at (-2.5,-2) {};
\node [basicnode] (v11) at (-0.5,-3) {};
\node [basicnode] (v12) at (-0.5,-4) {};
\node [basicnode] (v8) at (-4.5,-4) {};
\node [basicnode] (v7) at (-4.5,-3) {};


\draw [basicedge] (v7) edge (v8);
\draw [basicedge] (v8) edge (v9);
\draw [basicedge] (v9) edge (v7);
\draw [basicedge] (v9) edge (v10);
\draw [basicedge] (v9) edge (v11);
\draw [basicedge] (v9) edge (v12);
\draw [basicedge] (v12) edge (v11);

\draw [highlightededge] (v10) edge (v7);
\draw [highlightededge] (v10) edge (v8);
\draw [highlightededge] (v8) edge (v12);
\end{scope}



\begin{scope}[shift={(19,6.75)}]
\node [basicnode] (v9) at (-2.5,-3.5) {};
\node [basicnode] (v10) at (-2.5,-2) {};
\node [basicnode] (v11) at (-0.5,-3) {};
\node [basicnode] (v12) at (-0.5,-4) {};
\node [basicnode] (v8) at (-4.5,-4) {};
\node [basicnode] (v7) at (-4.5,-3) {};


\draw [basicedge] (v7) edge (v8);
\draw [basicedge] (v8) edge (v9);
\draw [basicedge] (v9) edge (v7);
\draw [basicedge] (v9) edge (v10);
\draw [basicedge] (v9) edge (v11);
\draw [basicedge] (v9) edge (v12);
\draw [basicedge] (v12) edge (v11);

\draw [highlightededge] (v11) edge (v7);
\draw [highlightededge] (v10) edge (v12);
\draw [highlightededge] (v10) edge (v11);
\end{scope}



\begin{scope}[shift={(15.5,4.25)}]
\node [basicnode] (v9) at (-2.5,-3.5) {};
\node [basicnode] (v10) at (-2.5,-2) {};
\node [basicnode] (v11) at (-0.5,-3) {};
\node [basicnode] (v12) at (-0.5,-4) {};
\node [basicnode] (v8) at (-4.5,-4) {};
\node [basicnode] (v7) at (-4.5,-3) {};


\draw [basicedge] (v7) edge (v8);
\draw [basicedge] (v8) edge (v9);
\draw [basicedge] (v9) edge (v7);
\draw [basicedge] (v9) edge (v10);
\draw [basicedge] (v9) edge (v11);
\draw [basicedge] (v9) edge (v12);
\draw [basicedge] (v12) edge (v11);

\draw [highlightededge] (v8) edge[bend right=25] (v11);
\draw [highlightededge] (v10) edge (v12);
\draw [highlightededge] (v10) edge (v11);
\end{scope}


\end{tikzpicture}


==> figures/lp_limits_intro_figure_vertical.tex <==
\begin{tikzpicture}[scale=0.8]

% Left side
\begin{scope}[shift={(1,-0.5)}]
\node [basicnode] (v4) at (-3.5,2.5) {};
\node [basicnode] (v2) at (-2,2.5) {};
\node [basicnode] (v5) at (-3,4) {};
\node [basicnode] (v6) at (-1.5,4) {};
\node [basicnode] (v1) at (-3.5,1) {};
\node [basicnode] (v3) at (-2,1) {};
\draw [basicedge] (v1) edge (v2);
\draw [basicedge] (v3) edge (v4);
\draw [basicedge] (v3) edge (v2);
\draw [basicedge] (v4) edge (v2);
\draw [basicedge] (v2) edge (v5);
\draw [basicedge] (v2) edge (v6);
\draw [basicedge] (v5) edge (v6);

\draw [highlightededge] (v5) edge (v4);
\draw [highlightededge] (v4) edge (v1);
\draw [highlightededge] (v1) edge (v3);
\end{scope}


\begin{scope}[shift={(1,-0.5)}]
\node [basicnode] (v9) at (-2.5,-3.5) {};
\node [basicnode] (v10) at (-2.5,-2) {};
\node [basicnode] (v11) at (-0.5,-3) {};
\node [basicnode] (v12) at (-0.5,-4) {};
\node [basicnode] (v8) at (-4.5,-4) {};
\node [basicnode] (v7) at (-4.5,-3) {};


\draw [basicedge] (v7) edge (v8);
\draw [basicedge] (v8) edge (v9);
\draw [basicedge] (v9) edge (v7);
\draw [basicedge] (v9) edge (v10);
\draw [basicedge] (v9) edge (v11);
\draw [basicedge] (v9) edge (v12);
\draw [basicedge] (v12) edge (v11);
\end{scope}

\node [blanknode] (v13) at (-4.5,-0.5) {};
\node [blanknode] (v14) at (1.5,-0.5) {};
\node [blanknode] (v15) at (1.5,5.5) {};
\node [blanknode] (v16) at (1.5,-5.5) {};
\draw [blanknode]  (v13) edge (v14);
\draw [blanknode]  (v15) edge (v16);

% Text nodes
\node [textnode] at (-1.5,5) {Original Graph with Three};
\node [textnode] at (-1.5,4.5) {Links to Remove};

\node [textnode] at (-1.5,-1) {Same Network with the Three};
\node [textnode] at (-1.5,-1.5) {Links Removed};

\node [textnode] at (4.5,5) {Valid Reconstructions};

% Right side
\begin{scope}[shift={(7,6)}]
\node [basicnode] (v9) at (-2.5,-3.5) {};
\node [basicnode] (v10) at (-2.5,-2) {};
\node [basicnode] (v11) at (-0.5,-3) {};
\node [basicnode] (v12) at (-0.5,-4) {};
\node [basicnode] (v8) at (-4.5,-4) {};
\node [basicnode] (v7) at (-4.5,-3) {};


\draw [basicedge] (v7) edge (v8);
\draw [basicedge] (v8) edge (v9);
\draw [basicedge] (v9) edge (v7);
\draw [basicedge] (v9) edge (v10);
\draw [basicedge] (v9) edge (v11);
\draw [basicedge] (v9) edge (v12);
\draw [basicedge] (v12) edge (v11);

\draw [highlightededge] (v10) edge (v7);
\draw [highlightededge] (v10) edge (v8);
\draw [highlightededge] (v8) edge (v12);
\end{scope}



\begin{scope}[shift={(7,2.75)}]
\node [basicnode] (v9) at (-2.5,-3.5) {};
\node [basicnode] (v10) at (-2.5,-2) {};
\node [basicnode] (v11) at (-0.5,-3) {};
\node [basicnode] (v12) at (-0.5,-4) {};
\node [basicnode] (v8) at (-4.5,-4) {};
\node [basicnode] (v7) at (-4.5,-3) {};


\draw [basicedge] (v7) edge (v8);
\draw [basicedge] (v8) edge (v9);
\draw [basicedge] (v9) edge (v7);
\draw [basicedge] (v9) edge (v10);
\draw [basicedge] (v9) edge (v11);
\draw [basicedge] (v9) edge (v12);
\draw [basicedge] (v12) edge (v11);

\draw [highlightededge] (v10) edge (v7);
\draw [highlightededge] (v10) edge (v12);
\draw [highlightededge] (v10) edge (v11);
\end{scope}



\begin{scope}[shift={(7,-0.5)}]
\node [basicnode] (v9) at (-2.5,-3.5) {};
\node [basicnode] (v10) at (-2.5,-2) {};
\node [basicnode] (v11) at (-0.5,-3) {};
\node [basicnode] (v12) at (-0.5,-4) {};
\node [basicnode] (v8) at (-4.5,-4) {};
\node [basicnode] (v7) at (-4.5,-3) {};


\draw [basicedge] (v7) edge (v8);
\draw [basicedge] (v8) edge (v9);
\draw [basicedge] (v9) edge (v7);
\draw [basicedge] (v9) edge (v10);
\draw [basicedge] (v9) edge (v11);
\draw [basicedge] (v9) edge (v12);
\draw [basicedge] (v12) edge (v11);

\draw [highlightededge] (v8) edge[bend right=25] (v11);
\draw [highlightededge] (v10) edge (v12);
\draw [highlightededge] (v10) edge (v11);
\end{scope}


\end{tikzpicture}
